Evaluating Explanation Methods for Multivariate Time Series Classification

Multivariate time series classification is an important computational task arising in applications where data is recorded over time and over multiple channels. For example, a smartwatch can record the acceleration and orientation of a person's motion, and these signals are recorded as multivariate time series. We can classify this data to understand and predict human movement and various properties such as fitness levels. In many applications classification alone is not enough, we often need to classify but also understand what the model learns (e.g., why was a prediction given, based on what information in the data). The main focus of this paper is on analysing and evaluating explanation methods tailored to Multivariate Time Series Classification (MTSC). We focus on saliency-based explanation methods that can point out the most relevant channels and time series points for the classification decision. We analyse two popular and accurate multivariate time series classifiers, ROCKET and dResNet, as well as two popular explanation methods, SHAP and dCAM. We study these methods on 3 synthetic datasets and 2 real-world datasets and provide a quantitative and qualitative analysis of the explanations provided. We find that flattening the multivariate datasets by concatenating the channels works as well as using multivariate classifiers directly and adaptations of SHAP for MTSC work quite well. Additionally, we also find that the popular synthetic datasets we used are not suitable for time series analysis.

==> experiments_v01.tex <==
\section{Experiments}
\label{sec:experiments}

As sketched before, in this work we used three different synthetic datasets and two real-world ones namely Counter Movement Jump (from now called CMJ) and Military Press (from now on called MP).

In order to have a wider set of possible experiments, we used one methodology to evaluate the explanations performances when the methods are applied to synthetic datasets, for which we can have ground truth labels and another one to evaluate the real-world dataset. 

In our experiments, we have compared dCAM as a proponent of the proper multivariate time series. We chose to do such a choice because among all the methods tailored for CNNs, dCAM relies on CAM which is very popular both in images and in time series explanations. As stressed in Section \ref{sec:rel_works} other than


In the rest of this section we are going to describe everything that was done in the same way for both dataset types and in Sections \ref{sec:exp_synth} and Section \ref{sec:realistic} the specific methodologies used.

\begin{figure}
    \centering
    %\includegraphics{}
    \subfloat[\label{fig:shap_chBych}]{\includegraphics[width=0.46\textwidth]{AALTD23-MVTS_Explanation/figs/shap_chBych.png} }
    \hspace{0.05\textwidth}
    \subfloat[\label{fig:shap_flatten}]{\includegraphics[width=0.4\textwidth]{AALTD23-MVTS_Explanation/figs/shap_flatten.png}  }
    \caption{Different strategies to use timeXpalin library in a multivariate scenario, supposing the number of channels $c=3$. In Figure \ref{fig:shap_chBych} $c$ different classifiers are trained one for each channel; explaining them will produce $c$ different heat maps of length $nS$: stacking all of them together the result is a matrix of dimension $c \times Ns $. In Figure \ref{fig:shap_flatten} the time series are flattened and one single classifier is trained using the concatenated channel. Explaining the classifier using a number of segments $ c \times nS$ is possible to reshape the resulting vector into a 2D matrix having the same shape as in the previous case.  }
    \label{fig:different_shap}
\end{figure}

Generally, the experiments aim to compare: 
\begin{itemize}
    \item SHAP explanation applied to Rocket followed by a Logistic Regression. For this purpose, we use the \textit{sktime} library \cite{loning2019sktime} to implement Rocket, \textit{scikit-learn} \cite{scikit-learn} for Logistic Regression and \textit{TimeXpain} \cite{mujkanovic2020timexplain} to apply SHAP.
    \\ Using this library is possible to divide the time series into segments so that SHAP will quantify the importance of consecutive time points rather than single ones; anyway it is only possible to explain univariate time series: supposing the series have a length of $ts$ time points, $c$ channels and the number of segments chosen is $nS$, we use two different strategies to apply TimeXplain to multivariate time series as illustrated in Figure \ref{fig:different_shap}:

    
    \begin{itemize}
        \item \textit{channel by channel scenario}: train one classifier for each channel and explain each of them. This will result in heat map vectors having $nS$ element each representing how much was important this specific segment in the classification. Stacking together all the $c$ vectors obtained by the $c$ classifiers, the result is a matrix of shape $c \times nS$.
        
        %\item \textit{channel by channel scenario}: trained one classifier for each channel in a dataset: for each of them, the heat map produced will be a vector of $nS$ values, each of these representing how much the corresponding channel segment was important for the model output. Stacking together all the $c$ vectors obtained by the $c$ classifiers, the result is a matrix of shape $c \times nS$.
    
        \item \textit{flatten dataset scenario}: trained a single classifier using the dataset fatten version in which all the columns are concatenated one after the other. In this case the number of chunks used was $c \times nS$ so that is possible to reshape this vector into a matrix having the same dimensions as before for comparison purposes.
    \end{itemize}

    
    \item dCAM explanation applied to dResNet classifier. Using this pair we can apply directly both dResNet and dCAM as they can natively support multivariate time series: the saliency map produced is a matrix of shape $c \times ts$ (differently from timeXplain, dCAM doesn't divide the series into segments) describing how much was important every time points in every channel for the classification.

    \item dResNet flatten for real-world experiments \#TBC
    
    \item plain Ridge Classifier: the datasets were flattened resulting in a single vector of dimension  $ c \times ts $ (same scenario as SHAP flatten dataset) before training the ridge Classifier. The learned weights represent the explanations. 
\end{itemize}

We have compared in total 4 different pairs  in our experiments: the two strategies for ROCKET/SHAP, dCAM/dResNet and Ridge Regression.

In Table \ref{tab:original_accuracies} we reported the accuracies of the best lassifiers for each dataset: all the experiments were done using a machine with 32 RAM GB, intel i7-12700H and nvidia GeForce RTX 350 Ti (the GPU was used only for dResNet/dCAM)

\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        dataset  &  dResNet & dResNet flatten  & rocket & rocket flatten & ridge classifier\\
        \hline
        Pesudo periodic & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        \hline
        Guassian & 0.83 & 0.89 & 0.93 & 0.72 & 1.0\\
        \hline
        Auto-Regressive & 0.82 & 0.81 & 0.87 & 0.73 & 1.0\\
         \hline
        Military press & 0.79 & 0.68 & 0.83 &  0.88 & 0.61 \\
        \hline
        CMJ & 0.82 & 0.91 &  0.87 & 0.83 & 0.44 \\
        \hline
    \end{tabular}
    \caption{Model accuracies}
    \label{tab:original_accuracies}
\end{table}

\subsection{Synthetic data}
\label{sec:exp_synth}

Each of the synthetic datasets has 100 instances both in train and test sets; each time series has a length of 100 time points and 20 different channels. All the datasets were built such that the discriminative part (consisting of an offset of $+1$ for the positive instances and $-1$ for the negative ones) ranges for time points in the interval $[10,20]$ and for channels in $[0,10]$ meaning that the $10\%$ of all time points and the $50\%$ of channels are discriminative.

Speaking about used parameters, for Rocket we performed a cross-validation to train the Logistic Regression using 5 folds and allowing up to 1000 iterations. 
\\ For dResNet we used the standard architecture with 64 filters, we trained using the Cross-Entropy Loss and Adam optimizer with a learning rate set to $0.00001$.
\\Finally for Ridge Classifier we used the standard scikit-learn parameters for a cross-validation using 5 folds.
\\ Regarding the explanation methods we used $10$ segments for timeXplain in the channel by channel scenario and consequentially $200$ segments in the flatten scenario, for dCAM the number of permutations $K$ to evaluate was set to $200$ and for the Ridge Classifier we took the learnt weights as the explanation.

It is very interesting to notice in Table \ref{tab:original_accuracies} that the best classifier for all three synthetic datasets is the ridge Classifier. This is strong evidence that these popular benchmark datasets, at least using these settings, aren't suitable for time series

\begin{figure}
    \centering
    %\includegraphics{}
    \subfloat[\label{fig:repeat_items}]{\includegraphics[width=0.42\textwidth]{AALTD23-MVTS_Explanation/figs/repeat_items.png} }
    \hspace{0.05\textwidth}
    \subfloat[\label{fig:average_items}]{\includegraphics[width=0.42\textwidth]{AALTD23-MVTS_Explanation/figs/average_items.png}  }
    \caption{ Two possible ways to reduce heat maps produced by different explanation methods to the same shape. In Figure \ref{fig:repeat_items} we take an element in the heat map produced by timeXplain repeating it 10 times. In Figure \ref{fig:average_items} we take 10 consecutive items produced by dCAM or Ridge averaging them into a single item}
    \label{fig:same_shape}
\end{figure}

In order to apply our methodology we need first of all to have the same dimension for all the heat maps: the ones produced by dCAM and Ridge have shape of $ c \times ts = 20 \times 100 $ while the ones by timeXplain have dimensions of $ c \times nS = 20 \times 10$.
\\ The only possible two ways to have the same shape are illustrated in Figure \ref{fig:same_shape}: either to repeat $10$ times each element in the SHAP explanations, so that every heat maps have dimension $ c \times ts = 20 \times 100 $ or to average 10 consecutive elements of dCAM and Ridge explanations into one single number so that all heat maps have shape $ c \times nS = 20 \times 10$. We have chosen the second option as we empirically verify all the metrics for these last two methods have a boost while the metrics for SHAP are the same as before 

Once we have the same shape for all the heat maps produced we have instantiated a ground truth matrix $GT$ for each dataset. 
\\ For the settings described before, this is a binary matrix that has a shape of $ c \times nS = 20 \times 10 $, all the elements are 0 but for the ones in $GT[1,0:10]$: in other words, this is a matrix representing whether the segment analyzed are important for the classification or not.
\\To be noted that the number of consecutive discriminative time points and channels, their range and the number of segments were chosen such that every segment has either only discriminative elements or only not discriminative ones. 

To metrics we used to compare the heat maps and the ground truth matrices were precision, recall, f1-score, PR-AUC and ROC-AUC.
Before computing these metrics all the heat maps produced for a single time series were rescaled in the range $[0,100]$ using mix-max normalization.

For precision, recall and f1 scores we had to fix a threshold: we chosed the medium value between $0$ and $100$ i.e. $50$. Each element that has a value higher than this threshold is considered important while every value lower was considered unimportant.
\\On the other hand PR-AUC and ROC-AUC are meant to not fix any threshold since they average multiple scores using different metrics into one single value.
\\ All these metrics computed for the 3 synthetic datasets are reported in Table \ref{tab:synth_metrics} 
\\ (-better to split into 3 different tables each one for a single dataset?)
\\ (to comment about the dataset types, no suitable for TS here?)


\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        dataset  & method  & precision & recall & f1 & PR-AUC & ROC-AUC & time to explain \\
        \hline
        pesudo periodic & shap ch-by-ch & 0.14 & 0.5 & 0.22 & 0.99 & 0.99 & 6.2 hr \\
        \hline
        pesudo periodic & shap concat & 0.21 & 0.5 & 0.29 & 0.94 & 0.99 & 3.5 hr \\
        \hline
        pesudo periodic & dCAM & 0.50 & 0.5 & 0.50 & 0.63 & 0.98 & 50 m \\
        \hline
        pesudo periodic & ridge & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0 s  \\
        \hline


        gaussian & shap ch-by-ch & 0.30 & 0.45 & 0.36 & 0.08 & 0.19 & 6.2 hr   \\
        \hline
        gaussian & shap concat & 0.05 & 0.47 & 0.09 & 0.05 & 0.30 & 3.5 hr \\
        \hline
        gaussian & dCAM & 0.35 & 0.15 & 0.21 & 0.35 & 0.94  & 50 m \\
        \hline
        gaussian & ridge & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0 s \\
        \hline

        auto regressive & shap ch-by-ch & 0.28 & 0.5 & 0.36 & 0.70 & 0.86 & 6.2 hr   \\
        \hline
        auto regressive & shap concat & 0.03 & 0.56 & 0.06 & 0.10 & 0.62 & 3.5 hr\\
        \hline
        auto regressive & dCAM & 0.33 & 0.15 & 0.21 & 0.06 & 0.57  & 50 m \\
        \hline
        auto regressive & ridge & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0 s \\
        \hline

    \end{tabular}
    \caption{ Scores and time spent for synthetic datasets: hrs stands for hours, ms stands for minutes and s stand for second}
    \label{tab:synth_metrics}
\end{table}

#TODO comments on these results

\subsection{Real-world data}
\label{sec:realistic}
%In these experiments, the only hyper-parameter changed was the number of filters for dResNet which is now set to 128 as we found slightly better results.
In these experiments, we used same different hyper-parameters compared to the last section: dResNet number of filters that are now set to $128$ because we empirically found better classification results; the number of dCAM permutation $K$ was set to $6$ for dCAM (this dataset has 3 channels so the number of possible channel permutations is just 6) while it was still $200$ for MP.
\\Finally we set the number of TimeXplain segments using the flattened dataset to $30$ and $80$ respectively for CMJ and MP to have the number of segments in this scenario equal to $ c \times nS $.
 
As skatched before, we used a different methodology for the real-world datasets for which we don't have any ground truth. 
\\Looking at the accuracies found in Table \ref{tab:original_accuracies} we can notice how for the two real-world datasets, the accuracies achieved by dResNet and Rocket are comparable or even better when they worked using the flattened dataset versions. Specifically, dResNet using CMJ has a gain of $0.09$ and Rocket gains $0.044$ points with MP using the flattened versions while for CMJ they are still comparable ($0.034$ worst).
That's why we decided to use the flatten version and the methodology developed by.....Trang that's your point!


\newpage
differences synt vs real-world datasets (gt vs perturbation)
- result using realistic datasets

\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        dataset  &  dResNet & rocket concat & min Rocket channel-wise & max Rocket channel-wise \\
        \hline
        CMJ & 0.82 & 0.877 prev ( 0.865) & 0.787 & 0.849 \\
        \hline
        military press & 0.79 & 0.831 prev (0.833) & 0.359 & 0.596 \\
        \hline
    \end{tabular}
    \caption{Accuracies of models used in the experiments}
    \label{tab:accuracies}
\end{table}

%MP:

 %RShoulder_Y was 0.48739495798319327 (595, 161)

 %RElbow_Y was 0.5966386554621849 (595, 161)

 %RWrist_Y was 0.5815126050420169 (595, 161)

 %LShoulder_Y was 0.519327731092437 (595, 161)

 %LElbow_Y was 0.5983193277310924 (595, 161)

%LWrist_Y was 0.5714285714285714 (595, 161)

%Hip_Y was 0.3596638655462185 (595, 161)

%LHip_Y was 0.3915966386554622 (595, 161)



%CMJ:

%channel 0
%CMJ accuracy on channel dim_0 was 0.7877094972067039 (179, 596)

%channel 1
%CMJ accuracy on channel dim_1 was 0.8491620111731844 (179, 596)

%channel 2
%CMJ accuracy on channel dim_2 was 0.8100558659217877 (179, 596)


==> experiments_v02.tex <==
\section{Experiments}
\label{sec:experiments}

%As sketched before, in this work we used three different synthetic datasets and two real-world ones namely Counter Movement Jump (from now called CMJ) and Military Press (from now on called MP).

%In order to have a wider set of possible experiments, we used one methodology to evaluate the explanations performances when the methods are applied to synthetic datasets, for which we can have ground truth labels and another one to evaluate the real-world dataset. 

%In our experiments, we have compared dCAM as a proponent of the proper multivariate time series. We chose to do such a choice because among all the methods tailored for CNNs, dCAM relies on CAM which is very popular both in images and in time series explanations. 
%The other methods are some univariate ones adapted to provide a multivariate explanation.


%In the rest of this section we are going to describe everything that was done in the same way for both dataset types and in Sections \ref{sec:exp_synth} and Section \ref{sec:realistic} the specific methodologies used.

In our experiments we aim to understand the strengths and weaknesses of existing methods for explaining multivariate time series classification.
For this purpose, we select and compare 4 different explanation methods chosen due to their popularity and effectiveness:
\begin{enumerate}
\item dCAM, one of the recent bespoke MTSC explanation methods we found in the literature. It was shown to outperform other existing explanation methods derived from deep learning models, including the popular CAM method. It is extracted from the dResNet classifier.

\item SHAP, a very popular method for explaining images and univariate time series. It can be applied post-hoc to any classifier.
%It is known for providing useful explanations, 
We apply SHAP to the ROCKET classifier.

\item RIDGE, a baseline intrinsic explainable classifier. This explanation method uses the learned weights from the Ridge Regression classifier. This method disregards the time ordering of data points.

\item RANDOM, an explanation method that uses saliency weights sampled uniformly at random. This serves as a lower bound on the quality of any explanation method.

\end{enumerate}
%\\On the other hand, all the other methods are meant for univariate time series and adapted to provide a multivariate explanation.

%Generally this work's aim is to compare these two types of explanation methods, evaluating the strong and the weak points of each of them in terms of explanation quality, time consumed, model agnostic vs model specific, etc.
Assuming the time series has length $L$ (number of time points) and $c$ channels, in our experiments we compare the following specific implementations:
\begin{itemize}

   \item dCAM explanation applied to dResNet classification. The saliency map produced is a matrix of shape $c \times L$ with an item at position $i,j$ describing how important the value at time $j$ in the channel $i$
  is. 
    \item SHAP explanation applied to Rocket (with a Logistic Regression classifier instead of Ridge, due to the availability of probability output for each classification instance). We have used the \textit{sktime} library \cite{loning2019sktime} to implement Rocket, \textit{scikit-learn} \cite{scikit-learn} for Logistic Regression and \textit{TimeXpain} \cite{mujkanovic2020timexplain} for SHAP applied to univariate time series classification.
    Using this library it is possible to divide the time series into segments so that SHAP will quantify the importance of consecutive time points: we have chosen to use 10 segments for each channel.
     %rather than single ones; anyway it is only possible to explain univariate time series: supposing the series have a length of $ts$ time points, $c$ channels and the number of segments chosen is $nS$, we use two different strategies to apply TimeXplain to multivariate time series as illustrated in Figure \ref{fig:different_shap}:
     To extract a multivariate explanation we applied two different strategies as shown in Figure \ref{fig:different_shap}.
     
    \begin{itemize}
        \item \textit{channel-by-channel}: train one classifier for each channel and explain each channel-classifier. This will result in heat map vectors having $10$ elements each, representing how  important was the segment in the classification. Stacking together all the $c$ vectors obtained by the $c$ classifiers, the result is a matrix of shape $c \times 10$. Differently from \cite{babayev2021interpreting}, to classify one single multivariate time series instance we relied on an ensemble model built from the single channel classifiers.
        
        %\item \textit{channel by channel scenario}: trained one classifier for each channel in a dataset: for each of them, the heat map produced will be a vector of $nS$ values, each of these representing how much the corresponding channel segment was important for the model output. Stacking together all the $c$ vectors obtained by the $c$ classifiers, the result is a matrix of shape $c \times nS$.
    
        \item \textit{concatenated dataset}: first concatenate all the channels to a single univariate time series, then train a single univariate classifier. In this case, the number of segments used was $c \times 10$ so that it is possible to reshape  the vector into a matrix having the same dimensions as the previous case.
        \end{itemize}
        
    \item plain Ridge Classifier: we used the concatenated dataset (same scenario as before) in which all the time series have a length of $ c \times L$. The learned weights by the classifier represent the explanation.

    \item The Random explanation is obtained using $U(0,100)$ sampling to obtain a $c \times L$ matrix with random weights.
\end{itemize}

We note that by reshaping the explanations provided by each method to a 2D matrix, we can have the same structure for both the method providing a 2D heat map directly as is the case for dCAM, and for methods that produce a 1D vector for the explanations, as is the case for SHAP channel-by-channel, SHAP applied to the concatenated dataset or Ridge.

\begin{figure}
    \centering
    %\includegraphics{}
    \subfloat[\label{fig:shap_chBych}]{\includegraphics[width=0.45\textwidth]{AALTD23-MVTS_Explanation/figs/shap_chBych.png} }
    \hspace{0.05\textwidth}
    \subfloat[\label{fig:shap_flatten}]{\includegraphics[width=0.45\textwidth]{AALTD23-MVTS_Explanation/figs/shap_flatten.png}  }
    \caption{Different strategies to use the timeXplain library in a multivariate scenario, for $c=3$. Different classifiers are trained one for each channel. For explaining each classifier, $c$ different heat maps of length $10$ are produced: stacking these vectors together results in a matrix of dimension $c \times 10$ (Fig \ref{fig:shap_chBych}). In Fig \ref{fig:shap_flatten} the time series are concatenated and one single classifier is trained. We explain the classifier using a number of segments $c \times 10$ and reshape the resulting vector into a 2D matrix having the same shape as in the previous case.}
    \label{fig:different_shap}
\end{figure}
%(that's why for the last one we selected as segment numbers $c \times 10$, so that it has the same number of total items compared to SHAP channel-by-channel)
%We have compared in total 4 different pairs  in our experiments: the two strategies for ROCKET/SHAP, dCAM/dResNet and Ridge Regression.
All the experiments were done using a machine with 32GB RAM, Intel i7-12700H CPU and a Nvidia GeForce RTX 350 Ti GPU (the GPU was used only for training dResNet/dCAM).
All the code used to perform the experiments is available on a Github repository\footnote{\url{https://anonymous.4open.science/r/ECML_PKDD_2023-795A}}.


\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        Dataset  &  dResNet & dResNet concat  & Rocket & Rocket concat & RidgeCV\\
        \hline
        Pseudo-Periodic & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 \\
        
        Gaussian & 0.83 & 0.89 & 0.93 & 0.72 & 1.0\\
        
        Auto-Regressive & 0.82 & 0.81 & 0.87 & 0.73 & 1.0\\
         \hline
        Military Press & 0.79 & 0.68 & 0.83 &  0.88 & 0.61 \\
        
        CMJ & 0.82 & 0.91 &  0.87 & 0.83 & 0.44 \\
        \hline
    \end{tabular}
    \caption{Accuracy of evaluated classifiers in the multivariate setting, as well as the univariate setting after concatenating all the channels. The first 3 datasets are synthetic and the last 2 are real-world datasets.}
    \label{tab:original_accuracies}
\end{table}

\subsection{Synthetic Data}
\label{sec:exp_synth}

Before diving into the explanations for each dataset, we first take a look at the accuracy of classifiers that are used for producing the explanations.
In Table \ref{tab:original_accuracies} we report the accuracy of each classifier and  each dataset, for both the original multivariate dataset, as well as the concatenated dataset where all the channels were concatenated toghether to create univariate time series.
We note that all the classifiers have high accuracy, with RidgeCV doing particularly well on the synthetic datasets and Rocket being more accurate than dResNet across all datasets. We also note that for Military Press, concatenating all the channels hurts dResNet, but leads to improved accuracy for Rocket. For CMJ, the behavior is reversed, with dResNet showing a noticeable 9 percentage points improvement on the concatenated dataset, while Rocket loses 4 percentage points in accuracy.

For the synthetic data, we used the Rocket transform and performed cross-validation to train Logistic Regression using 5 folds and allowing up to 1000 iterations.  For dResNet we used 64 filters, and we trained using the Cross-Entropy Loss and Adam optimizer with a learning rate set to $0.0001$. Finally for RidgeCV we used the standard scikit-learn parameters for cross-validation using 5 folds.
Regarding the explanation methods we used $10$ segments for timeXplain in the channel-by-channel scenario and $200$ segments in the concatenated scenario, for dCAM the number of permutations to evaluate $k$ was set to $200$. %and for the Ridge Classifier we took the learnt weights as the explanation.

%It is very interesting to notice in Table \ref{tab:original_accuracies} that the best classifier for all three synthetic datasets is the ridge Classifier. This is strong evidence that these popular benchmark datasets, at least using these settings, aren't suitable for time series
%\begin{figure}
%    \centering
    %\includegraphics{}
%    \subfloat[\label{fig:repeat_items}]{\includegraphics[width=0.42\textwidth]{AALTD23-MVTS_Explanation/figs/repeat_items.png} }
%    \hspace{0.05\textwidth}
%    \subfloat[\label{fig:average_items}]{\includegraphics[width=0.42\textwidth]{AALTD23-MVTS_Explanation/figs/average_items.png}  }
%    \caption{ Two possible ways to reduce heat maps produced by different explanation methods to the same shape. In Figure \ref{fig:repeat_items} we take an element in the heat map produced by timeXplain repeating it 10 times. In Figure \ref{fig:average_items} we take 10 consecutive items produced by dCAM or Ridge averaging them into a single item}
%    \label{fig:same_shape}
%\end{figure}

The steps done for syntethic data evaluation are illustrated in Figure \ref{fig:synthetic_steps}.
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{AALTD23-MVTS_Explanation/figs/synthetic_steps.png}
    \caption{Steps performed in the synthetic data evaluation supposing we are comparing just 2 explanations. Step 1 is to reshape all the explanations so that they all have the same shape. After this step, all the explanations are rescaled in the range $[0,100]$. In Step 2 we instantiate the same ground truth matrix for all the datasets and compare this matrix against the reshaped and rescaled explanations. Finally in Step 3 we compute the desired metrics for each method and for each dataset.}
    \label{fig:synthetic_steps}
\end{figure}
The first step is to reshape all the explanations  so that they all have the same dimension. As using timeXplain we set the length of the segments to 10, we chose to average 10 consecutive elements for dCAM and Ridge explanation as we empirically saw  that all the metrics had a slight improvement. The alternative was to repeat 10 times the same item in SHAP explanations.
Once having the same shape, all the explanations were individually rescaled in the range $[0,100]$ for homogeneity.

%In order to apply our methodology we need first of all to have the same dimension for all the heat maps: the ones produced by dCAM and Ridge have shape of $ c \times n = 20 \times 100 $ while the ones by timeXplain have dimensions of $ c \times \text{n. segments} = 20 \times 10$.
%\\ The only possible two ways to have the same shape are illustrated in Figure \ref{fig:same_shape}: either to repeat $10$ times each element in the SHAP explanations %, so that every heat maps have dimension $ c \times ts = 20 \times 100 $ 
%or to average 10 consecutive elements of dCAM and Ridge explanations into one single number.
%so that all heat maps have shape $ c \times nS = 20 \times 10$. 
%We have chosen the second option as we empirically verify all the metrics for these last two methods have a boost while the metrics for SHAP are unchanged.

The second step is to instantiate a ground truth matrix $G$ and compare each explanation against it. For the settings described before, this is a binary matrix having shape $ 20 \times 10 $ (same dimension of explanations), all the elements are set to 0 but for the ones in $G[0:10,1]$ that are set to $1$. In other words, this is a binary matrix representing whether the segment analyzed are important for the classification or not.
\\To be noted that the number of consecutive informative time points and channels, their range and the number of segments were chosen such that every segment has either only informative elements or only not informative ones. 

The third and last point is to compute the used metrics for the evaluation i.e.,  Precision, Recall, F1-score, PR-AUC and ROC-AUC \cite{}.
\\For precision, recall and f1 scores, we had to fix a threshold dividing the values considered uninformative from the ones considered informative: we have chosen $50$ as the medium value between $0$ and $100$.
On the other hand PR-AUC and ROC-AUC are meant to not fix any threshold as they average multiple scores using different metrics into one single value.
All these metrics computed for the 3 synthetic datasets are reported in Table \ref{tab:synth_metrics}.

\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        Dataset  & Method  & Precision & Recall & F1 & PR-AUC & ROC-AUC & Explanation time \\\hline
        
        Pseudo-Periodic & shap ch-by-ch & 0.14 & 0.5 & 0.22 & 0.99 & 0.99 & 6.2 hr \\
        
        Pseudo-Periodic & shap concat & 0.21 & 0.5 & 0.29 & 0.94 & 0.99 & 3.5 hr \\
       Pseudo-Periodic & dCAM & 0.50 & 0.5 & 0.50 & 0.63 & 0.98 & 50 m \\

       Pseudo-Periodic & ridge & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0 s  \\
        \hline

        Gaussian & shap ch-by-ch & 0.30 & 0.45 & 0.36 & 0.08 & 0.19 & 6.2 hr   \\
        
        Gaussian & shap concat & 0.05 & 0.47 & 0.09 & 0.05 & 0.30 & 3.5 hr \\
        
        Gaussian & dCAM & 0.35 & 0.15 & 0.21 & 0.35 & 0.94  & 50 m \\
        
        Gaussian & ridge & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0 s \\
        \hline

        auto regressive & shap ch-by-ch & 0.28 & 0.5 & 0.36 & 0.70 & 0.86 & 6.2 hr   \\
        
        auto regressive & shap concat & 0.03 & 0.56 & 0.06 & 0.10 & 0.62 & 3.5 hr\\
        
        auto regressive & dCAM & 0.33 & 0.15 & 0.21 & 0.06 & 0.57  & 50 m \\
        
        auto regressive & ridge & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0 s \\
        \hline

        All   \ & random & 0.05 & 0.5 & 0.09 & 0.05 & 0.5 & 0 s\ \\
        \hline

    \end{tabular}
    \caption{ Scores and time spent for synthetic datasets: hrs stands for hours, ms stands for minutes and s stand for seconds}
    \label{tab:synth_metrics}
\end{table}





\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        Dataset  & Method  & Precision & Recall & F1 & PR-AUC & ROC-AUC & Explanation time \\\hline
        
        Pseudo-Periodic & shap ch-by-ch & 0.73 & 0.94 & 0.82 & 0.99 & 0.99 & 6.2 hr \\
        
        Pseudo-Periodic & shap concat & 0.92 & 0.66 & 0.77 & 0.99 & 0.99 & 3.5 hr \\
        
       Pseudo-Periodic & dCAM & 0.50 & 0.5 & 0.50 & 0.63 & 0.98 & 50 m \\

       Pseudo-Periodic & ridge & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0 s  \\
        \hline

        Gaussian & shap ch-by-ch & 0.88 & 0.63 & 0.73 & 0.91 & 0.99 & 6.2 hr   \\
        
        Gaussian & shap concat & 0.34 & 0.18 & 0.24 & 0.16 & 0.71 & 3.5 hr \\
        
        Gaussian & dCAM & 0.36 & 0.15 & 0.21 & 0.35 & 0.94  & 50 m \\
        
        Gaussian & ridge & 0.83 & 1.0 & 0.9 & 1.0 & 1.0 & 0 s \\
        \hline

        auto regressive & shap ch-by-ch & 0.85 & 0.60 & 0.71 & 0.49 & 0.77 & 6.2 hr   \\
        
        auto regressive & shap concat & 0.27 & 0.13 & 0.18 & 0.29 & 0.57 & 3.5 hr\\
        
        auto regressive & dCAM & 0.34 & 0.15 & 0.21 & 0.06 & 0.57  & 50 m \\
        
        auto regressive & ridge & 1.0 & 1.0 & 1.0 & 1.0 & 1.0 & 0 s \\
        \hline

        All   \ & random & 0.05 & 0.5 & 0.09 & 0.05 & 0.5 & 0 s\ \\
        \hline

    \end{tabular}
    \caption{ Scores and time spent for synthetic datasets: hrs stands for hours, ms stands for minutes and s stand for seconds}
    \label{tab:new_synth_metrics}
\end{table}

Looking at these results it is possible to note that all the time ridge Classifier has perfect metrics. These results along with the one provided in Table \ref{tab:original_accuracies} (perfect accuracies of ridge for the 3 synthetic datasets), are very strong evidence that these commonly used benchmarks are not ideal for time series analyses at least using the parameters described before. 

Comparing dCAM with SHAP it is very difficult to find a clear winner among them as dCAM has every time a better recall while SHAP has a precision greater or equal to dCAM. Looking at the Areas under the curve, for pseudo periodic the two methods have similar results for ROC but a better value for PR by SHAP, looking at the Gaussian dataset dCAM has far better results while focusing on the auto-regressive dataset SHAP is the best one.

Another point to notice is that some scores are comparable or even lower than what is expected by a random method. 
Finally, the time elapsed for the explanations is remarkable: 50 minutes for dCAM, 3.5 hours for SHAP flatten scenario, and more than 6 hours for SHAP channel by channel.

\subsection{Real-world Data}
\label{sec:realistic}
%In these experiments, the only hyper-parameter changed was the number of filters for dResNet which is now set to 128 as we found slightly better results.
In this section we used some different hyper-parameters: dResNet number of filters is now set to $128$ because we empirically found better classification results; the number of dCAM permutations $k$ was set to $6$ for dCAM (this dataset has 3 channels so the number of possible channel permutations is just 6) while it is still $200$ for MP.
We set the number of timeXplain segments using the concatenated dataset to $30$ for CMJ and $80$ for MP so that they are still equal to $ c \times 10 $.

%As sketched before, we used a different methodology for the real-world datasets for which we don't have any ground truth. 
Looking at the accuracies found in Table \ref{tab:original_accuracies} we can notice how for the two real-world datasets, the accuracies achieved by dResNet and Rocket are comparable or even better when using the concatenated dataset versions. Specifically, dResNet using CMJ has a gain of $0.09$ and Rocket gains $0.044$ points with MP using the concatenated versions while for CMJ they are still comparable ($0.034$ worst).
That's why we decided to use the concatenated version and the methodology developed by \cite{nguyen2023amee} to evaluate the explanation methods.

\subsubsection{Evaluation of Explanation Methods.} We apply AMEE \cite{nguyen2023amee}, an explanation evaluation method for univariate time series classification task, on the CMJ and MP univariate datasets obtained through concatenating all channels. This method aims to measure the faithfulness of an explanation by estimating its impact on a set of independent classifiers (the \textit{referee classifiers}). If an explanation correctly points out the important areas of an univariate time series, perturbation of such areas will lead to a drop in accuracies of the referee classifiers. The faithfulness of the explanation is then calculated using the Area Under the Curve (AUC) of the accuracy drop curves of each referee classifiers. AMEE is designed to be robust by employing various perturbation strategies (i.e. how an important areas is perturbed and replaced with a new value) and a diverse set of high-performing referee classifiers.

For our task, we use the default perturbation strategies presented in the paper with three referee classifiers: MrSEQL \cite{le2019interpretable}, ROCKET \cite{dempster2020rocket}, and WEASEL 2.0 \cite{Schafer2023WEASELClassification}. Table \ref{tab:accuracies-ref} shows the accuracy of these referee classifiers on the evaluated datasets. The result of the evaluation is presented in Table \ref{tab:AMEE_CMJ} and Table \ref{tab:AMEE_MP} for CMJ and MP, respectively.

\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        dataset  &  MrSEQL & ROCKET & WEASEL 2.0 \\
        \hline
        CMJ & 0.76 & 0.88  & 0.92 \\
        \hline
        MP & 0.82 & 0.84 & 0.80 \\
        \hline
    \end{tabular}
    \caption{Accuracy of referee classifiers in AMEE evaluation}
    \label{tab:accuracies-ref}
\end{table}



\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|c}
        \hline
        XAI method & average scaled AUC & scaled ranking & explanation power & rankig \\
        \hline
        shap concat & 0.29 & 0.00 & 1.00 & 1 \\
        \hline
        random & 0.30 & 0.01 & 0.99 & 2 \\
        \hline
        dCAM & 0.45 & 0.61 & 0.39 & 3 \\
        \hline
        shap channelByChannell & 0.53 & 0.95 & 0.05 & 4 \\
        \hline
        ridge & 0.55 & 1.00 & 0.0 & 5 \\
        \hline
    \end{tabular}
    \caption{Results of AMEE method applied on CMJ}
    \label{tab:AMEE_CMJ}
\end{table}

\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        XAI method & average scaled AUC & scaled ranking & explanation power & rankig \\
        \hline
        shap concat & 0.05 & 0.00 & 1.00 & 1 \\
        \hline
        dCAM & 0.56 & 0.67 & 0.33 & 2 \\
        \hline
        random & 0.76 & 0.93 & 0.07 & 3 \\
        \hline
        ridge & 0.82 & 1.00 & 0.0 & 4 \\
        \hline
    \end{tabular}
    \caption{Results of AMEE method applied on MP}
    \label{tab:AMEE_MP}
\end{table}



\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        dataset  &  dResNet & rocket concat & min Rocket channel-wise & max Rocket channel-wise \\
        \hline
        CMJ & 0.82 & 0.877 prev ( 0.865) & 0.787 & 0.849 \\
        \hline
        military press & 0.79 & 0.831 prev (0.833) & 0.359 & 0.596 \\
        \hline
    \end{tabular}
    \caption{Accuracies of models used in the experiments}
    \label{tab:accuracies}
\end{table}


%MP:

 %RShoulder_Y was 0.48739495798319327 (595, 161)

 %RElbow_Y was 0.5966386554621849 (595, 161)

 %RWrist_Y was 0.5815126050420169 (595, 161)

 %LShoulder_Y was 0.519327731092437 (595, 161)

 %LElbow_Y was 0.5983193277310924 (595, 161)

%LWrist_Y was 0.5714285714285714 (595, 161)

%Hip_Y was 0.3596638655462185 (595, 161)

%LHip_Y was 0.3915966386554622 (595, 161)



%CMJ:

%channel 0
%CMJ accuracy on channel dim_0 was 0.7877094972067039 (179, 596)

%channel 1
%CMJ accuracy on channel dim_1 was 0.8491620111731844 (179, 596)

%channel 2
%CMJ accuracy on channel dim_2 was 0.8100558659217877 (179, 596)

